Real-world K-Anonymity Applications: the \textsc{KGen} approach and its evaluation in Fraudulent Transactions

K-Anonymity is a property for the measurement, management, and governance of the data anonymization. Many implementations of k-anonymity have been described in state of the art, but most of them are not able to work with a large number of attributes in a "Big" dataset, i.e., a dataset drawn from Big Data. To address this significant shortcoming, we introduce and evaluate \textsc{KGen} an approach to K-anonymity featuring Genetic Algorithms. \textsc{KGen} promotes such a meta-heuristic approach since it can solve the problem by finding a pseudo-optimal solution in a reasonable time over a considerable load of input. \textsc{KGen} allows the data manager to guarantee a high anonymity level while preserving the usability and preventing loss of information entropy over the data. Differently from other approaches that provide optimal global solutions catered for small datasets, \textsc{KGen} works properly also over Big datasets while still providing a good-enough solution. Evaluation results show how our approach can still work efficiently on a real world dataset, provided by Dutch Tax Authority, with 47 attributes (i.e., the columns of the dataset to be anonymized) and over 1.5K+ observations (i.e., the rows of that dataset), as well as on a dataset with 97 attributes and over 3942 observations.

==> chapters/9_acknowledgements.tex <==
\section{Acknowledgements} \label{sec:ack}
This work has been sponsored by the West-Brabant-Zeeland Taskforce that fights subversive and organized crime exploiting data science, AI and Big data technologies. The experiments that have been described in this article have been anonymized themselves to avoid any conflicts with AVG/GDPR.

==> chapters/front_page.tex <==
\begin{titlepage}
	\centering
	\includegraphics[width=.9\linewidth]{figures/jads-logo-rgb_3_orig.png}\par\vspace{1cm}
	
	{\huge\bfseries DELIVERABLE TASKFORCE WEST-BRABANT \& ZEELAND - JADS: SMART CELL FINDING THE MONEY \par}
	\vspace{2cm}
	{\Large\itshape Daniel \textsc{De Pascale}\\}
	\vspace{0.8cm}
	{\Large\itshape Willem-Jan \textsc{van den Heuvel}\\}
	\vspace{0.8cm}
	{\Large\itshape Giuseppe \textsc{Cascavilla}\\}
	\vspace{0.8cm}
	{\Large\itshape Damian \textsc{A. Tamburri}\\}
	\vfill
	%supervised by \par
	%professeurs EC \textsc{Martigny}


% Bottom of the page
	{\large \today\par}
\end{titlepage}

\newpage

==> figures/img/generalization_age.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, trim={0, 3cm, 0, 0}]{figures/img/generalization_age1.png}
    \caption{Generalization hierarchy of age}
    \label{fig:gen_AGE}
\end{figure}

==> figures/img/generalization_postcode.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, trim={0, 3cm, 0, 0}]{figures/img/generalization_postcode3.png}
    \caption{Generalization hierarchy of a postcode}
    \label{fig:gen_ZIP}
\end{figure}

==> figures/img/genetic_algorithm_flow_chart.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/img/genetic_algorithm_flow_chart.png}
    \caption{Genetic algorithm flow chart}
    \label{fig:ga_flow_chart}
\end{figure}

==> figures/img/lattice_reducted.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{figures/img/lattice_reducted.png}
    \caption{Example of lattice reducted, with <2, 1, 0> as new starting node}
    \label{fig:lattice_reducted}
\end{figure*}

==> figures/img/singlepoint_crossover.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width = .8\linewidth]{figures/img/singlepoint_crossover3.png}
    \caption{\footnotesize Example of single point crossover, applied on two parent in order to generate two new children. The point is used to split the values, so the first part of parent1 and the last part of parent2 begin the first children, instead the last part of parent1 and the first part of parent2 begin the second children.}
    \label{fig:singlepoint_crossover}
\end{figure}

==> formula/eqBracket.tex <==
\begin{equation}
    eq_{i, j} = \left\{
    \begin{matrix}
        1 & if \quad QI_{i}(A_{k}) = QI_{j}(A_{k}), & \forall k = 1,...,M \\
        0 & otherwise & 
    \end{matrix}\right.
\end{equation}


==> formula/kanon.tex <==
\begin{equation}
    \sum_{j=1}^{N} eq_{i, j} \geq k \quad \forall\; i = 1,...,N
\end{equation}

==> formula/kanon_sum.tex <==
\begin{equation}
    \sum_{j=1}^{N} eq_{i, j} \geq k \quad \forall\; i = 1,...,N
\end{equation}


==> formula/lattice_size.tex <==
\begin{equation} \label{eqn:lattice_size}
    latticeSize \ = \ \prod_{i = 0}^{N} \\\ (maxLOG_{i} - minLOG_{i}) + 1
\end{equation}

==> pseudocode/kgen2.tex <==
\begin{algorithm}
    \caption{KGEN}
    \label{kgen_PSEUDOCODE2}
    \begin{algorithmic}[1]
        \Procedure{KGEN}{}
        \State \text{minNode, maxNode = LatticePreprocessing()}
        \State $P_{i} \gets \text{Generate starting population}$
        \State \text{Evaluate $P_{i}$}
        \While {$currentEvaluation < maxEvaulations$}
            \State $\text{offsprings} \gets \text{Inizialize offsprings array}$
            \For {$i=0$ to $populationSize/2$}
	    		\State $\text{Select two parents from } P_{i}$
	    		\State \text{Generate offspring solutions via crossover}
	    		\State \text{Mutate offspring solutions}
	    		\State \text{Evaluate offspring solutions}
	    		\State \text{Add offspring solutions to offsprings array}
    		\EndFor
    		\State \textbf{end for}
    		\State \text{Add offsprings to $P_{i}$}
    		\State $P_{i+1} \gets survivalSelection(P_{i}$
        \EndWhile
        \State \textbf{end while}
        %\If {$i > \textit{stringlen}$} \Return false
        %\EndIf
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> pseudocode/kgen_crossover.tex <==
\begin{algorithm}[b]
    \caption{KGEN Crossover Operator}
    \label{alg: kgen_crossover_PSEUDOCODE}
    \begin{algorithmic}[1]
        \Procedure{KGEN Crossover }{Solution parent1, Solution parent2}
        \State $offsprings \gets \text{initialize offsprings array solutions}$
        \State $\text{minLatticeNode} = \text{minValues(parent1, parent2)}$
        \State $\text{maxLatticeNode} = \text{maxValues(parent1, parent2)}$
        
		\If{\text{both of parents are k-anonymized}}
		    \If{\text{minLatticeNode is k-anonymized}}
		        \State \text{add minLatticeNode to the offsprings}
		    \Else
    		    \State $\text{add random nodes between minLatticeNode} \linebreak \text{\qquad \qquad \ \ and both of parents}$
		    \EndIf
		\ElsIf{\text{both of parents are not k-anonymized}}
		    \State \text{add maxLatticeNode to the offsprings}
		\Else
		    \If{\text{parent1 is k-anonymized}}
    		    \State $\text{add random node between minLatticeNode} \linebreak \text{\qquad \qquad \ \ and parent1 to the offsprings}$
		    \Else
		        \State $\text{add random node between minLatticeNode} \linebreak \text{\qquad \qquad \ \ and parent2 to the offsprings}$
		    \EndIf
		\EndIf
		\State \text{\textbf{return} offsprings}
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> results/F2_results.tex <==
\begin{figure*}[t]
\centering
%\begin{adjustbox}{minipage=\linewidth,scale=0.6}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expTime_F2.png}
  \caption{Execution time}
  \label{fig:execution_time_f2}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_F2.png}
  \caption{Accuracy}
  \label{fig:accuracy_f2}
\end{subfigure}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expLog_F2.png}
  \caption{Level of generalization}
  \label{fig:log_f2}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expSupp_F2.png}
  \caption{Level of suppression}
  \label{fig:suppression_f2}
\end{subfigure}
\caption{Results}
\label{fig:results_f2}
%\end{adjustbox}
\end{figure*}

==> results/LD_results.tex <==
\begin{figure*}[t]
\centering
%\begin{adjustbox}{minipage=\linewidth,scale=0.6}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expTime_LD.png}
  \caption{Execution time}
  \label{fig:execution_time_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_LD.png}
  \caption{Accuracy}
  \label{fig:accuracy_ld}
\end{subfigure}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expLog_LD.png}
  \caption{Level of generalization}
  \label{fig:log_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expSupp_LD.png}
  \caption{Level of suppression}
  \label{fig:suppression_ld}
\end{subfigure}
\caption{Results}
\label{fig:results_ld}
%\end{adjustbox}
\end{figure*}

==> results/accuracy.tex <==
\begin{figure*}[t]
\centering
%\begin{adjustbox}{minipage=\linewidth,scale=0.6}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_LD_cut.png}
  \caption{Accuracy on c2k dataset}
  \label{fig:acc_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_F2.png}
  \caption{Accuracy on real dataset}
  \label{fig:acc_f2}
\end{subfigure}
\caption{Accuracy}
\label{fig:acc}
%\end{adjustbox}
\end{figure*}

==> results/suppression.tex <==
\begin{figure*}[ht]
\centering
%\begin{adjustbox}{minipage=\linewidth,scale=0.6}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expSupp_LD.png}
  \caption{Level of suppression of c2k dataset}
  \label{fig:sup_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expSupp_F2.png}
  \caption{Level of suppression of real dataset}
  \label{fig:sup_f2}
\end{subfigure}
\caption{Level Of Suppression}
\label{fig:sup}
%\end{adjustbox}
\end{figure*}

==> results/time_acc.tex <==
\begin{figure*}[t]
\centering
%\begin{adjustbox}{minipage=\linewidth,scale=0.6}
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expTime_LD.png}
  \caption{\footnotesize Execution time c2k dataset.}
  \label{fig:execution_time_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expTime_F2.png}
  \caption{\footnotesize Execution time real dataset.}
  \label{fig:execution_time_f2}
\end{subfigure}
\caption{\footnotesize Execution time evaluation results over the considered datasets.}
\label{fig:execution_time}



\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_LD.png}
  \caption{\footnotesize Accuracy on c2k dataset.}
  \label{fig:acc_ld}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=.95\linewidth]{results/expAccuracy_F2.png}
  \caption{\footnotesize Accuracy on real dataset.}
  \label{fig:acc_f2}
\end{subfigure}
\caption{\footnotesize Accuracy evaluation results over the considered datasets.}
\label{fig:acc}
%\end{adjustbox}
\end{figure*}

==> tables/accuracyF2.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    
    \begin{tabular}{l|llll}
        \hline
        & Exp 1 & Exp 2 & Exp 3 & Exp 4 \\
        \hline
        EXHAUSTIVE & 1.0 & 1.0 & - & - \\
        OLA & 1.0 & 1.0 & 1.0 & - \\
        KGEN & 1.0 & 0.98 & 0.72 & - \\
        RANDOM & 0.2 & 0.11 & 0.14 & - \\
        \hline
    \end{tabular}
    
    \vspace{0.3cm}
    \caption{\textit{Accuracy comparison}}
    \label{tab:accuracyF2}
\end{table}

==> tables/crossover_table.tex <==
\begin{table}[th]
\renewcommand{\arraystretch}{1.5}
\footnotesize
\resizebox{\linewidth}{!}{
    \begin{center}
        \begin{tabular}{ccccc}
            \hline
            \\
            Parents & K-ANON & MIN/MAX & K-ANON & Offspring \\
            \\
            \hline
            Parent 1 & V & MIN & ? & S \\
            Parent 2 & V & MAX & V & S \\
            \hline
            Parent 1 & V & MIN & F & S \\
            Parent 2 & F & MAX & V & S \\
            \hline
            Parent 1 & F & MIN & F & S \\
            Parent 2 & V & MAX & V & S \\
            \hline
            Parent 1 & F & MIN & F & S \\
            Parent 2 & F & MAX & ? & S \\
            \hline
        \end{tabular}
    \end{center}
}
\vspace{1em}

\caption{\textit{Original dataset. The attribute Name is an Identifier. Instead Age, Gender and Postcode are Quasi-Identifiers}}
\label{tab:Table1}
\end{table}

==> tables/dataset.tex <==
\begin{table}[th]
    \subfloat[caption]{
    \begin{tabular}{ccccc}
        \hline
        \\
        Name & Age & Gender & Postcode & Crime \\
        \\
        \hline
        \\
        Alice & 25 & F & 80015 & Assault \\
        Max & 28 & M & 80019 & Kidnapping \\
        Bob & 42 & M & 85073 & Homicide  \\
        Frank & 49 & M & 85071 & Rape \\ 
        \\
        \hline
    \end{tabular}
    \\\\
    \caption{\textit{Dataset k-anonymized. Considering the QI, the number of indistinguishable rows are two. So, the dataset is k-anonymized (k = 2)}}
    \label{tab:Table1}    
    }

    \subfloat[caption]{
    \begin{tabular}{ccccc}
        \hline
        \\
        Name & Age & Gender & Postcode & Crime \\ 
        \\
        \hline
        \\
        ***** & 20 - 30 & P & 8001* & Assault \\
        ***** & 20 - 30 & P & 8001* & Kidnapping \\
        \\
        ***** & 40 - 50 & P & 8507* & Homicide  \\
        ***** & 40 - 50 & P & 8507* & Rape \\ 
        \\
        \hline
    \end{tabular}
    }
    \\\\

\caption{\textit{Dataset k-anonymized. Considering the QI, the number of indistinguishable rows are two. So, the dataset is k-anonymized (k = 2)}}
\label{tab:Table2}

\end{table}

==> tables/datasetExampleKANON.tex <==
\begin{table}[!t]
\begin{center}
\renewcommand{\arraystretch}{1.5}
\label{tab:dataset_table_anonymized}
\footnotesize
\caption{\footnotesize Dataset k-anonymized. Considering the QI, the number of indistinguishable rows are two. So, the dataset is k-anonymized (k = 2).}
\resizebox{.5\linewidth}{!}{
        \begin{tabular}{ccccc}
            \hline
            Name & Age & Gender & Postcode & Crime \\
            \hline
            ***** & 20 - 30 & P & 8001* & Assault \\
            ***** & 20 - 30 & P & 8001* & Kidnapping \\
            ***** & 40 - 50 & P & 8507* & Homicide  \\
            ***** & 40 - 50 & P & 8507* & Rape \\
            \hline
        \end{tabular}
}
\end{center}
\end{table}

==> tables/executionTimeF2.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|llll}
        \hline
        & Exp 1 & Exp 2 & Exp 3 & Exp 4 \\
        \hline
        EXHAUSTIVE & 0.297 & 4.969 & - & - \\
        OLA & 0.235 & 4.35 & 428.392 & - \\
        KGEN & 0.158 & 3.915 & 141.271 & 389.039 \\
        RANDOM & 0.069 & 4.085 & 156.563 & 546.755 \\
        \hline
    \end{tabular}
    \vspace{0.3cm}
    \caption{\textit{Execution time comparison}}
    \label{tab:execTimeF2}
\end{table}

==> tables/experimental_setup.tex <==
\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \resizebox{.6\linewidth}{!}{
        \begin{tabular}{l|llll}
            \hline
            & min k-value & Attributes & Rows & QID \\
            \hline
            c2k & 2 & 98 & 3942 & [3..10, 15, 20, 25] \\
            F$^2$ & 2 & 47 & 1599 & [3..10, 15, 20, 25] \\
            \hline
        \end{tabular}
    }
    \caption{\footnotesize Experimental setup.}
    \label{tab:experimental_setup}
\end{table}

==> tables/f2InfoExp.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.5}
\footnotesize
\resizebox{\linewidth}{!}{
    \begin{tabular}{llll}
        \hline
        \textbf{Attribute name} & \textbf{Type} & \textbf{LOG} & \textbf{Experimentation} \\
        \hline
        Date & DATE & 2 & Exp 1, 2, 3, 4 \\
        HouseNr & INT & 4 & Exp 1, 2, 3, 4 \\
        HouseLet & STRING & 3 & Exp 1, 2, 3, 4 \\
        HouseCode & STRING & 3 & Exp 2, 3, 4 \\
        Postcode & STRING & 7 & Exp 2, 3, 4 \\
        Place & PLACE & 2 & Exp 3, 4 \\
        PhoneNumber & STRING & 10 & Exp 3, 4 \\
        MobileNumber & STRING & 0 & Exp 3, 4 \\
        KvkNumber & STRING & 8 & Exp 3, 4 \\
        VestigingsNumber & STRING & 12 & Exp 3, 4 \\
        Rsin & STRING & 9 & Exp 4 \\
        BtwNumber & STRING & 14 & Exp 4 \\
        IbanNumber & STRING & 0 & Exp 4 \\
        Facebook & STRING & 96 & Exp 4 \\
        PnNumber & STRING & 21 & Exp 4 \\
        \hline
    \end{tabular}
}

\vspace{0.3cm}

\caption{\textit{This table shows the information about all the quasi-identifiers attributes used in all the experimentation done in the case study, together with their type and their level of generalization (LOG)}}
\label{tab:f2InfoExp}


\end{table}

==> tables/kgenParameters.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \resizebox{.8\linewidth}{!}{
        \begin{tabular}{ll}
            \hline
            \multicolumn{2}{l}{KGEN Paramenters} \\
            \hline
            Population size & 100 \\
            Max evaluations & 5000 \\
            Crossover probability & 0.9 \\
            Mutation probability & 0.2 \\
            Horizontal mutation probability & 0.4 \\
            \hline
        \end{tabular}
    }
    
    \vspace{0.3cm}
    \caption{\textit{Settings of genetic algorithm}}
    \label{tab:kgen_paramenters}
    \vspace{-0.4cm}
\end{table}



==> tables/logF2.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|llll}
        \hline
        & Exp 1 & Exp 2 & Exp 3 & Exp 4 \\
        \hline
        EXHAUSTIVE & 0.33 & 0.42 & - & - \\
        OLA & 0.33 & 0.42 & 0.52 & - \\
        KGEN & 0.33 & 0.43 & 0.63 & 0.73 \\
        RANDOM & 0.89 & 0.93 & 0.95 & 0.87 \\
        \hline
    \end{tabular}
    \vspace{0.3cm}
    \caption{\textit{LOG comparison}}
    \label{tab:logF2}
\end{table}

==> tables/selection_k_anonymity.tex <==
\begin{figure}[!h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \resizebox{.6\linewidth}{!}{%
        \begin{tabular}{cccc}
            \hline
            \textbf{Solution} & \textbf{KLEV} & \textbf{LOG} & \textbf{Percentage} \\
            \hline
            1 & 2 & 0.69 & 0.06 \\
            2 & 3 & 0.85 & 0.1 \\
            3 & 2 & 0.56 & 0.06 \\
            4 & 2 & 0.72 & 0.06 \\
            5 & 2 & 0.61 & 0.06 \\
            6 & 3 & 0.44 & 0.1 \\
            7 & 3 & 0.55 & 0.1 \\
            8 & 2 & 0.85 & 0.06 \\
            9 & 110 & 0.8 & 0.4 \\
            \hline
        \end{tabular}
        %\caption{Solutions with their K-Anonymity level and their probability to be chosen}
    }
    \resizebox{.6\linewidth}{!}{%
        \begin{tabular}{c}
             \\
            \begin{tikzpicture}
                \pie [color={black!10, black!30, black!50}]{30/K=2, 30/K=3, 40/K=110}
            \end{tikzpicture} \\
             \\
        \end{tabular}
        %\caption{Pie chart representing probabilities for all of K-Anonymity values of a single Selection process}
    }
    
    \caption{\textit{Selection process based on K-Anonymity metric. In the table are showed the solutions with their K-Anonymity level and their probability to be chosen. The pie chart, instead, represents probabilities to choose a pool of solutions, given the K-Anonymity value chosen in this selection process}}
    \label{fig:selection_k-anonymity}
\end{figure}

==> tables/sizeProblemF2.tex <==
\begin{table}[h]
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|llll}
        \hline
        & \textbf{Exp 1} & \textbf{Exp 2} & \textbf{Exp 3} & \textbf{Exp 4} \\
        \hline
        \textbf{N. of nodes} & $6*10^1$ & $1.9*10^3$ & $7.4*10^6$ & $2.4*10^{12}$ \\
        \textbf{N. of QI} & $3$ & $5$ & $10$ & $15$ \\
        \hline
    \end{tabular}
    \vspace{0.3cm}
    \caption{\textit{Lattice size of the real dataset, for all the experimentation take into account}}
    \label{tab:f2_size}
\end{table}

==> tables/sizeProblemLD.tex <==
\begin{table}[b]
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|llll}
        \hline
        & \textbf{Exp 1} & \textbf{Exp 2} & \textbf{Exp 3} & \textbf{Exp 4} \\
        \hline
        \textbf{N. of nodes} & $2.1*10^2$ & $5.4*10^3$ & $1.4*10^5$ & $1.34*10^{17}$ \\
        \textbf{N. of QI} & $3$ & $5$ & $10$ & $25$ \\
        \hline
    \end{tabular}
    \vspace{0.3cm}
    \caption{\textit{Lattice size for c2k\_data\_comma.csv, for all the experimentation take into account}}
    \label{tab:ld_size}
\end{table}

==> tables/suppression_f2.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{l|llll}
        \hline
        & Exp 1 & Exp 2 & Exp 3 & Exp 4 \\
        \hline
        EXHAUSTIVE & 0.37\% & 0.37\% & - & - \\
        OLA & 0.37\% & 0.37\% & 0.36\% & - \\
        KGEN & 0.37\% & 0.37\% & 0.3\% & 0.31\% \\
        RANDOM & 0.31\% & 0.1\% & 0.1\% & 0.24\% \\
        \hline
    \end{tabular}
    \vspace{0.3cm}
    \caption{\textit{Suppression comparison}}
    \label{tab:suppression_f2}
\end{table}
